Adaptive Contrastive Decoding in Retrieval-Augmented Generation for Handling Noisy Contexts

When using large language models (LLMs) in knowledge-intensive tasks, such as open-domain question answering, external context can bridge the gap between external knowledge and the LLMs' parametric knowledge. Recent research has been developed to amplify contextual knowledge over the parametric knowledge of LLMs with contrastive decoding approaches. While these approaches could yield truthful responses when relevant context is provided, they are prone to vulnerabilities when faced with noisy contexts. We extend the scope of previous studies to encompass noisy contexts and propose adaptive contrastive decoding (ACD) to leverage contextual influence effectively. ACD demonstrates improvements in open-domain question answering tasks compared to baselines, especially in robustness by remaining undistracted by noisy contexts in retrieval-augmented generation.

==> Sections/Note.tex <==


% intro -> related works 

With the objective of closely adhering to the context provided, 
context-augmented generation strategies have been developed to better utilize the context and produce more factual and context-relevant responses at the inference time \citep{zhou-etal-2023-context, he2024rest}.
% [2] Context faithful decoding methods
Especially, approaches integrated with contrastive decoding \citep{li-etal-2023-contrastive, malkin-etal-2022-coherence, liu-etal-2021-dexperts} yield significant enhancement by amplifying the influence of the given context at decoding step \citep{shi2023trusting, zhao2024enhancing}. % CD 설명?
% the generation of outputs within the given context
% such as summarization and open-domain question answering,
These context-aware contrastive decoding methods with the objective of generating responses faithful to the given context show effective performance in summarization \citep{see2017point, narayan-etal-2018-dont}, knowledge flipping \citep{longpre2022entitybased}, and question answering with gold contexts.


% TODO
1. 방법론 이름, 논문 이름 확정
그래야 figure 도 다시 그릴수있음

2. 현수오빠가 써준 intro 내꺼랑 합치고
conclusion 안고침 고쳐야함
limitation 써야함

3. 첨부터 쭉 읽어보고 한번 더 고치고
figure 다시 다 그리고

4. main table 어케하고 (모델 어떤거 main table 에서 쓸껀지) 분량 보고
